TIRAMISU: A Polyhedral Compiler for Dense and Sparse Deep Learning

In this paper, we demonstrate a compiler that can optimize sparse and recurrent neural networks, both of which are currently outside of the scope of existing neural network compilers (sparse neural networks here stand for networks that can be accelerated with sparse tensor algebra techniques). Our demonstration includes a mapping of sparse and recurrent neural networks to the polyhedral model along with an implementation of our approach in TIRAMISU, our state-of-the-art polyhedral compiler. We evaluate our approach on a set of deep learning benchmarks and compare our results with hand-optimized industrial libraries. Our results show that our approach at least matches Intel MKL-DNN and in some cases outperforms it by 5x (on multicore-CPUs).

==> tex/acknowledgement.tex <==
%\vspace{-0.25cm}
\section{Acknowledgement}
This work was supported by the Applications Driving Architectures (ADA) Research Center, a JUMP Center co-sponsored by SRC (Semiconductor Research Corporation) and DARPA.
